Smartphone Security Behavioral Scale: A New Psychometric Measurement for Smartphone Security

Despite widespread use of smartphones, there is no measurement standard targeted at smartphone security behaviors. In this paper we translate a well-known cybersecurity behavioral scale into the smartphone domain and show that we can improve on this translation by following an established psychometrics approach surveying 1011 participants. We design a new 14-item Smartphone Security Behavioral Scale (SSBS) exhibiting high reliability and good fit to a two-component behavioural model based on technical versus social protection strategies. We then demonstrate how SSBS can be applied to measure the influence of mental health issues on smartphone security behavior intentions. We found significant correlations that predict SSBS profiles from three types of MHIs. Conversely, we are able to predict presence of MHIs using SSBS profiles.We obtain prediction AUCs of 72.1% for Internet addiction,75.8% for depression and 66.2% for insomnia.

==> 45_survey_items.tex <==
\begin{table*}[!ht]
\centering
\caption{List of questions of smartphone security behaviors generated by security professionals}
\label{table3}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llll}
ID & Item & $\mu$ & $\sigma$ \\
\hline
A1 & I turn off WiFi on my smartphone when not actively using it. & 2.88 & 1.38 \\
A2 & I perform banking transactions/operations on my smartphone while connected to a public network. & 3.62 & 1.35 \\
A3 & I connect to public WiFi using my smartphone. (R) & 2.92 & 1.78 \\
A4 & I use a Virtual Private Network (VPN) app while connected to a public network. & 2.43 & 1.38 \\
A5 & When downloading an app, I check that the app is from the official/expected source. & 3.92 & 1.07 \\
A6 & Before downloading a smartphone app I ensure the download is from official application stores (e.g. Apple App Store, GooglePlay, Amazon Appstore) & 4.04 & 1.08 \\
A7 & I manually revoke permissions from apps. & 3.15 & 1.11 \\
A8 & I grant smartphone apps the permissions they request. (r) & 2.56 & 0.89 \\
A9 & I disable geotagging of images captured by smartphone's camera app. & 3.17 & 1.39 \\
A10 & I check which apps are running in the background. & 3.59 & 1 \\
A11 & I delete apps I don't frequently use. & 3.88 & 0.97 \\
A12 & I enable two-step authentication when offered by an app. & 3.45 & 1.15 \\
A13 & I reset my Advertising ID on my smartphone. & 2.32 & 1.36 \\
A14 & I check my smartphone's privacy settings. & 3.5 & 1.06 \\
A15 & I turn off location services on my smartphone when I am not actively using them & 3.41 & 1.28 \\
A16 & I turn off bluetooth (NFC, wifi) on my smartphone when I am not actively using it & 3.67 & 1.32 \\
A17 & I use an anti-virus app & 2.72 & 1.53 \\
A18 & I store proprietary business information on my smartphone. (R) & 3.7 & 1.33 \\
A19 & I store personal health information on my smartphone. (R) & 3.52 & 1.39 \\
A20 & I verify the recipient/sender before sharing text messages or other information using smartphone apps & 3.71 & 1.14 \\
A21 & I use an adblocker on my smartphone. & 2.84 & 1.48 \\
A22 & I pay attention to the pop-ups on my smartphone when connecting it to another device (e.g. laptop, desktop). & 3.83 & 1.07 \\
A23 & I care about the source of the app when performing financial and/or shopping tasks on that app & 4.05 & 0.98 \\
A24 & I back-up my smartphone's contacts, photos and videos on another device/cloud & 3.44 & 1.23 \\
A25 & I delete any online communications (i.e., texts, emails, social media posts) that look suspicious & 3.92 & 1.11 \\
A26 & I get permissions from my friends before sharing them on a photo or video online & 3.48 & 1.24 \\
A27 & I check the latest news updates regarding my smartphone and apps & 3.36 & 1.09 \\
A28 & I use private browsing on my smartphone. & 3.06 & 1.16 \\
A29 & I use biometrics (fingerprint, face recognition) to unlock my smartphone. & 3.07 & 1.61 \\
A30 & I enable encrypted storage (or phone memory) on my smartphone. & 2.87 & 1.48 \\
A31 & I use a rooted/jailbroken phone (r). & 1.97 & 1.35 \\
A32 & I turn on the ``lost my device'' feature on my smartphone. & 2.89 & 1.53 \\
A33 & I use a password/passcode to unlock my smartphone. & 3.87 & 1.27 \\
A34 & I hide device in my smartphone's bluetooth settings. & 2.63 & 1.43 \\
A35 & I use a privacy screen on my smartphone & 2.58 & 1.51 \\
A36 & I manually cover my smartphone's screen when using it in the public area (e.g., bus or subway). & 2.89 & 1.25 \\
A37 & I change my password for online services/accounts using my smartphone. & 2.89 & 1.24 \\
A38 & I share my smartphone's passcode/PIN with other(s). (r) & 4 & 1.27 \\
A39 & I use password manager app to manage my passwords on my smartphone. & 2.55 & 1.48 \\
A40 & I store passwords and usernames on my smartphone. & 3.32 & 1.41 \\
A41 & I change my passcode/PIN for my smartphone's screen lock at a regular basis. & 2.7 & 1.31 \\
A42 & I use different passwords for different accounts that I have on my smartphone. & 3.68 & 1.14 \\
A43 & When I'm prompted about a software update on my smartphone, I install it as soon as I can & 3.53 & 1.09 \\
A44 & I make sure that the programs smartphone applications I use are up-to-date. & 3.79 & 1.05 \\
A45 & Before downloading a smartphone app I read its privacy policy to ensure my information is handled securely & 2.96 & 1.33 \\
\end{tabular}%
}
\end{table*}

==> Reference.tex <==
References
McKinley, R. K., Manku-Scott, T., Hastings, A. M., French, D. P., & Baker, R. (1997). Reliability and validity of a new measure of patient satisfaction with out of hours primary medical care in the United Kingdom: development of a patient questionnaire. Bmj, 314(7075), 193.

Piedmont R.L. (2014) Inter-item Correlations. In: Michalos A.C. (eds) Encyclopedia of Quality of Life and Well-Being Research. Springer, Dordrecht

Allen, M. J., & Yen, W. M. (2002). Introduction to measurement theory. Long Grove, IL: Waveland Press. 

Cohen, R. J., & Swerdlik, M. E. (2005). Psychological testing and assessment: An introduction to tests and measurement (6th ed.). New York: McGraw-Hill. 

Harbach, M., Von Zezschwitz, E., Fichtner, A., De Luca, A., & Smith, M. (2014). It’s a hard lock life: A field study of smartphone (un) locking behavior and risk perception. In 10th Symposium On Usable Privacy and Security ({SOUPS} 2014)(pp. 213-230).

Harbach, M., De Luca, A., & Egelman, S. (2016, May). The anatomy of smartphone unlocking: A field study of android lock screens. In Proceedings of the 2016 CHI Conference on Human Factors in Computing Systems (pp. 4806-4817). ACM.


Gascon, H., Uellenbeck, S., Wolf, C., & Rieck, K. (2014). Continuous authentication on mobile devices by analysis of typing motion behavior. Sicherheit 2014–Sicherheit, Schutz und Zuverlässigkeit.

Fisher, D., Dorner, L., & Wagner, D. (2012, October). Short paper: location privacy: user behavior in the field. In Proceedings of the second ACM workshop on Security and privacy in smartphones and mobile devices (pp. 51-56). ACM.

Wijesekera, P., Baokar, A., Hosseini, A., Egelman, S., Wagner, D., & Beznosov, K. (2015). Android permissions remystified: A field study on contextual integrity. In 24th {USENIX} Security Symposium ({USENIX} Security 15) (pp. 499-514).

Almuhimedi, H., Schaub, F., Sadeh, N., Adjerid, I., Acquisti, A., Gluck, J., ... & Agarwal, Y. (2015, April). Your location has been shared 5,398 times!: A field study on mobile app privacy nudging. In Proceedings of the 33rd annual ACM conference on human factors in computing systems (pp. 787-796). ACM.
Liang, H., & Xue, Y. (2010). Understanding security behaviors in personal computer usage: A threat avoidance perspective. Journal of the association for information systems, 11(7), 394-413.

Verkijika, S. F. (2018). Understanding smartphone security behaviors: An extension of the protection motivation theory with anticipated regret. Computers & Security, 77, 860-870.

Zhou, W., Zhou, Y., Jiang, X., & Ning, P. (2012, February). Detecting repackaged smartphone applications in third-party android marketplaces. In Proceedings of the second ACM conference on Data and Application Security and Privacy (pp. 317-326). ACM.

Muppavaram, K., Rao, M. S., Rekanar, K., & Babu, R. S. (2018). How Safe Is Your Mobile App? Mobile App Attacks and Defense. In Proceedings of the Second International Conference on Computational Intelligence and Informatics(pp. 199-207). Springer, Singapore.
Kang, J. M., Seo, S. S., & Hong, J. W. K. (2011, September). Usage pattern analysis of smartphones. In 2011 13th Asia-Pacific Network Operations and Management Symposium (pp. 1-8). IEEE.

Kulkarni, S. P., & Bojewar, S. (2015). Vulnerabilities of Smart Phones. International Research Journal of Engineering and Technology (IRJET), 2(9), 2422-2426.

Li, M., Meng, Y., Liu, J., Zhu, H., Liang, X., Liu, Y., & Ruan, N. (2016, October). When CSI meets public WiFi: Inferring your mobile phone password via WiFi signals. In Proceedings of the 2016 ACM SIGSAC Conference on Computer and Communications Security (pp. 1068-1079). ACM.

Kooistra, J. (2018). Newzoo’s 2018 Global Mobile Market Report: Insights into the World’s 3 Billion Smartphone Users. https://newzoo.com/insights/articles/newzoos-2018-global-mobile-market-report-insights-into-the-worlds-3-billion-smartphone-users/


==> method.tex <==
%METHOD
Our goal of this study is to develop a measurement to assess users' security behavioral intentions to comply with smartphone security advices recommended by security professionals. We conducted a two-phases online survey study. In the phase-1, we tested four dimensions of SeBIS developed by Egelman and Peer~\cite{egelman2015scaling}. According to our results, four dimensions of SeBIS may not be applicable to users' smartphone security behaviors. That is, users' security behaviors could be different from the general computer security behavior. Therefore, we conducted a phase-2 study to develop a new measurement for smartphone security behavior. 

For both phases of study, we recruited participants from the U.S. via Amazon Mechanical Turk. To ensure the quality of data, we put the attention-check questions in each section of the survey. The attention-check questions were randomly inserted in the questionnaire and had similar format to other questions. Participants were required to select the choice required in the statement (i.e., \textit{I go to grocery shopping on every Thursday. Please select `Never'}). We removed the responses from participants who failed answering attention-check questions. We next describe the details of study design and results for each phase of the study.

